Using Experiments to Correct for Selection in Observational Studies

Researchers increasingly have access to two types of data: (i) large observational datasets where treatment (e.g., class size) is not randomized but several primary outcomes (e.g., graduation rates) and secondary outcomes (e.g., test scores) are observed and (ii) experimental data in which treatment is randomized but only secondary outcomes are observed. We develop a new method to estimate treatment effects on primary outcomes in such settings. We use the difference between the secondary outcome and its predicted value based on the experimental treatment effect to measure selection bias in the observational data. Controlling for this estimate of selection bias yields an unbiased estimate of the treatment effect on the primary outcome under a new assumption that we term latent unconfoundedness, which requires that the same confounders affect the primary and secondary outcomes. Latent unconfoundedness weakens the assumptions underlying commonly used surrogate estimators. We apply our estimator to identify the effect of third grade class size on students outcomes. Estimated impacts on test scores using OLS regressions in observational school district data have the opposite sign of estimates from the Tennessee STAR experiment. In contrast, selection-corrected estimates in the observational data replicate the experimental estimates. Our estimator reveals that reducing class sizes by 25% increases high school graduation rates by 0.7 percentage points. Controlling for observables does not change the OLS estimates, demonstrating that experimental selection correction can remove biases that cannot be addressed with standard controls.

==> Section_2_excess_text_on_imputation_case_etc.tex <==

\iffalse
\subsection{A Binary Outcome Example}

Our key assumption is that there is a relationship between the short term and long term unobserved components $\alpha^\pp_i$ and $\alpha^\pp_i$ that allows us to remove the endogeneity bias in the long term relationship using the difference between the short term results for the experimental and observational data using a control function approach (\citet{heckman1985alternative, imbens2009identification, wooldridge2015control, kline2019heckits}). 

Randomization in the experimental sample implies that we can estimate the parameters of the model for the secondary outcome,  $\tau^\pps$ and $\gamma^\pps$,  using an ordinary least squares regression of $Y^\pps_i$ on $W_i$ and $X_i$.

Now consider the primary outcome. 
  
For the purpose of the first example in this section, we assume both the secondary and primary outcome are binary, $Y^\pp_i(w),Y^\pps_i(w)\in\{0,1\}$, for $w\in\{0,1\}$.
For expositional reasons we also assume in this section that there are no pretreatment variables.

For all outcome types  $t\in\{\pps,\pp\}$, all groups  $g\in\{\ppe,\ppo\}$, and all treatment levels  $w\in\{0,1\}$, define the averages $\oy^{t,g}_w$ and sample sizes
$N^g_w$:
\[ \oy^{t,g}_w\equiv \frac{1}{N^g_w}\sum_{i=1}^N Y^t_i \been_{G_i=g,W_i=w},
\hskip1cm {\rm and}\ \ 
N^g_w\equiv  \sum_{i=1}^N  \been_{G_i=g,W_i=w}.\]
Assuming that  $N^\ppo_0$, $N^\ppo_1$,  $N^\ppe_0$, and $N^\ppe_1$ are all positive, 
 six of the eight average outcomes $\oy^{t,g}_w$ can be calculated from the data,
$\oy^{\pp,\ppo}_0$, $\oy^{\pp,\ppo}_1$, $\oy^{\pps,\ppo}_0$, $\oy^{\pps,\ppo}_1$, $\oy^{\pps,\ppe}_0$, and $\oy^{\pps,\ppe}_1$. The remaining two, 
 $\oy^{\pp,\ppe}_0$ and $\oy^{\pp,\ppe}_1$  cannot be calculated because we do not observe the primary outcome in the experimental sample.

\subsubsection{Using the Two Samples Separately}

Let us first consider estimation of $\tau^\pp$ and $\tau^\pps$ using one sample at a time. Using only the experimental sample there is no way to estimate the average treatment effect on the primary outcome, because this sample does not contain any information on the primary outcome.  We can estimate the average effect on the secondary outcome, using the experimental sample, as
\[ \hat\tau^{\pps,\ppe}=\oy^{\pps,\ppe}_1-\oy^{\pps,\ppe}_0.\]
%=\frac{1}{N^\ppe_1}\sum_{i:G_i=\ppe,W_i=1} Y^\pps_i-\frac{1}{N^\ppe_0}\sum_{i:G_i=\ppe,W_i=0} Y^\pps_i,\hskip1cm
This estimator $\hat\tau^{\pps,\ppe}$ is unbiased for $\tau^\pps$ if the experimental sample has external validity and could be considered  a random sample from the population of interest (formally, if $G_i\indep (Y_i(0),Y_i(1))$, what \citet{hotz2005predicting} call location unconfoundedness). 


Using only the observational sample the natural estimator for the average causal effect on the primary and secondary outcomes would be
\[ \hat\tau^{\pp,\ppo}=\oy^{\pp,\ppo}_1-\oy^{\pp,\ppo}_0,\hskip1cm {\rm and}\ \ 
 \hat\tau^{\pps,\ppo}=\oy^{\pps,\ppo}_1-\oy^{\pps,\ppo}_0
%=\frac{1}{N^\ppo_1}\sum_{i:G_i=\ppo,W_i=1} Y^\pp_i-\frac{1}{N^\ppo_0}\sum_{i:G_i=\ppo,W_i=0} Y^\pp_i
,\]
respectively. For these estimators to be consistent for the average causal effect of the treatment on the primary and secondary outcomes we would need unconfoundedness, which, in the absence of pretreatment variables, corresponds to:
\[ W_i\ \indep\ \Bigl(Y^\pps_i(0),Y^\pps_i(0),Y^\pp_i(0),Y^\pp_i(0)\Bigr)\ \Bigr|\ G_i=\ppo.\]
With only the observational sample there is no alternative  for obtaining point estimates of the average treatment effect on the primary and secondary outcomes.

\subsubsection{Combining the Two Samples}

Now consider estimation of $\tau^\pps$ in the presence of both experimental and observational samples.  In this case we have two distinct estimators for $\tau^\pps$, nameley
$\hat\tau^{\pps,\ppe}$ and $\hat\tau^{\pps,\ppo}$.  If we find no significant difference between $\hat\tau^{\pps,\ppe}$ and $\hat\tau^{\pps,\ppo}$, then both would appear to be reasonable estimates. We might improve the precision of either estimator by combining them efficiently (along the lines of, for example, \citet{rosenman2018propensity, rosenman2020combining, kallus2020role}). However, if we find a substantial and statistically significant difference between the two,  we can infer that either  the assignment in the observational sample is not  random (unconfoundedness does not hold for the observational sample), or the experimental sample is not a random sample from the population of interest (no external validity).  In that case there may still be efficiency gains in combining the data, as discussed in \citet{rosenman2020combining}. However, in large samples the two estimators will converge to different limits. 

There is no information in the data to determine whether unconfoundedness in the observational sample, or external validity in the experimental sample, is violated.  Note that these assumptions  are of a very different nature. The researcher has to use {\it a priori} arguments to choose between $\hat\tau^{\pps,\ppe}$ and $\hat\tau^{\pps,\ppo}$ and the corresponding assumptions. Choosing for $\hat\tau^{\pps,\ppe}$ would imply being less concerned with the external validity of the experimental sample, whereas the choice for $\hat\tau^{\pps,\ppo}$ would imply that the internal validity of the observational study would be viewed as less of a concern. In many cases researchers have argued for the primacy of internal validity over external validity ({\it e.g.}, \citet{shadishcookcampbell, imbens2010}), though others have argued against that perspective ({\it e.g.}, \citet{manski2013public, deaton2010}). If one prefers $\hat\tau^{\pps,\ppo}$ (downplaying the concerns about internal validity of the observational sample), the natural estimator for $\tau^\pp$ is $\hat\tau^{\pp,\ppo}$, and there is little use for the experimental sample. However, if the researcher prefers $\hat\tau^{\pps,\ppe}$, the question arises how to estimate $\tau^\pp$.

The current paper is concerned with this question. We take the position that there is  an {\it a priori} preference for  $\hat\tau^{\pps,\ppe}$ over $\hat\tau^{\pps,\ppo}$, possibly after accounting for differences in covariate distributions to deal with some of the external validity concerns (\citet{hotz2005predicting}). Then we address the  main question of how to adjust the estimator $\hat\tau^{\pp,\ppo}$ to take into account the difference between $\hat\tau^{\pps,\ppo}$ and $\hat\tau^{\pps,\ppe}$. Conceptually there are multiple natural ways of doing so. We discuss three of these ways that are ultimately equivalent in large samples. The first  one is based on imputation of the missing primary outcomes in the experimental sample. The second one is  based on weighting the units in the observational sample. The third one is based on a control function approach. In this simple nonparametric case with binary outcomes the three approaches lead to identical point estimates . 

\subsubsection{Imputation}

The first approach is to take a missing data perspective on the primary $Y_i^\pp$ in the experimental sample and  impute these missing values using the observational 
sample. Consider  unit $i$ in the experimental sample with $W_i=w$ and $Y^\pps_i=y^\pps$. Assuming the missing data on $Y^\pp_i$  are missing at random ({\it e.g.,} \citet{rubin1976inference, little2019statistical, rubin2004multiple}) suggests using the distribution of $Y^\pp_i$ among units in the observational sample with $W_i=w$ and $Y^\pps_i=y^\pps$ to impute the missing values. If we are interested in estimating the average effect, we can just use the average value of $Y^\pp_i$ in this subsample (the part of the observational sample with $W_i=w$ and $Y^\pps_i=y^\pps$), equal to , as the imputed value.
Denote  this average value for all values of $y^\pps$ and $w$ by: 
\[ \oy^{\pp,\ppo}_{w,y^\pps}\equiv 
\sum_{i=1}^N \been_{G_i=\ppo, W_i=w,Y^\pps_i=y^\pps}Y^\pp_i
\Bigl/\sum_{i=1}^N \been_{G_i=\ppo, W_i=w,Y^\pps_i=y^\pps}.\]
The imputed value for $Y^\pp_i$ for  unit $i$ in the experimental sample is then the average of $Y^\pp_j$ in the 
observational sample over all units $j$  with the same treatment level, $W_j=W_i$, and the same value for the secondary outcome, $Y^\pps_j=Y^\pps_i$:
\[ \hat Y^\pp_i\quiv \oy^{\pp,\ppo}_{W_i,Y^\pps_i}.\]
Then the imputation estimator for $\tau^\pp$ is the difference in average imputed values in the experimental sample by treatment status, leading to the first estimator for $\tau^\pp$:
%\[ \hat\tau^{\pp,\imp}=\frac{1}{N^\ppe_1}\sum_{i:G_i=\ppe} W_i \hat Y^\pp_i-\frac{1}{N^\ppe_0}\sum_{i:G_i=\ppe} (1-W_i)\hat Y^\pp_i\]
\begin{equation}\label{imp}\hat\tau^{\pp,\imp}\equiv \frac{1}{N^\ppe_1}
\sum_{i:G_i=\ppe} W_i \oy^{\pp,\ppo}_{W_i,Y^\pps_i}
-\frac{1}{N^\ppe_0}\sum_{i:G_i=\ppe} (1-W_i) \oy^{\pp,\ppo}_{W_i,Y^\pps_i}
.\end{equation}

\subsubsection{Weighting}

The second approach to using the experimental secondary outcomes  is to reweight the observational sample (where we do observe the primary outcome) to resemble the experimental sample where there are no unobserved confounders. Consider the $N^\ppo_w$ units in the observational sample with $W_i=w$. The fraction of those treated units  in the observational study with secondary outcome $Y^\pps_i=1$ is $\hat p^{\pps,\ppo}_w=\sum_{i:G_i=\ppo,W_i=w} Y^\pps_i/\sum_{i:G_i=\ppo,W_i=w} 1$. The experimental study tells us this fraction would have been approximately
$\hat p^{\pps,\ppe}_w=\sum_{i:G_i=\ppe,W_i=w} Y^\pps_i/\sum_{i:G_i=\ppe,W_i=w} 1$, had the treatment  been randomly assigned. 
The comparison $\hat p^{\pps,\ppo}_w$ versus $\hat p^{\pps,\ppe}_w$ reflects on the possible violation of the unconfoundedness assumption in the observational sample.
We can give these units a weight $\lambda_{w,1}\equiv \hat p^{\pps,\ppe}_w/\hat p^{\pps,\ppo}_w$ to adjust for the bias stemming from such violations.
Similarly, units with treatment $W_i=w$ and $Y^\pps_i=0$ would be given a weight $\lambda_{w,0}\equiv (1-\hat p^{\pps,\ppe}_w)/(1-\hat p^{\pps,\ppo}_w)$. We then
 use these weights to estimate the average effect on the primary outcome as
the difference of weighted averages of the treated and control outcomes in the observational sample, leading to the second estimator:
\begin{equation}\hat\tau^{\pp,\weight}\equiv 
\frac{\sum_{G_i=\ppo} \lambda_{1,Y^\pps_i} W_i Y^\pp_i}{\sum_{G_i=\ppo} \lambda_{1,Y^\pps_i}W_i }
-\frac{\sum_{G_i=\ppo} \lambda_{0,Y^\pps_i}(1-W_i) Y^\pp_i}{\sum_{G_i=\ppo} \lambda_{0,Y^\pps_i} (1-W_i)}
.\end{equation}
Straightforward algebra shows that  the imputation and weighting estimators for $\tau$ are identical,
$\hat\tau^{\pp,\imp}=\hat\tau^{\pp,\weight}$.
This algebraic result relies on the outcome model and the weights being fully nonparametric in this  example with the secondary outcome taking on only two values. In settings with the secondary outcome continuous, the imputation and weighting approaches will generally give different answers in finite samples.

%Excess Text from Control Function section
%For this we only need the data from the experimental sample.
 %In other words, the conditional mean of $Y^\pps_i$ given $W_i$ and $X_i$ has a causal interpretation as a function of $W_i$ in the experimental sample. 
 We cannot do this in the observational sample because of the potential correlation between $W_i$ and $ \alpha_i^\pps$.
 
%A key external validity condition is is captured by conditional independence of $\alpha_i$ and $G_i$ given covariates: \[\alpha_i^\pps\  \perp\!\!\!\perp\ G_i\ \Bigl|\ X_i.\]

\fi

%Such a correlation would imply that a linear regression of $Y^\pp_i$ on $W_i$ and $X_i$ using the data from the observational sample would not be consistent for the causal effect $\tau^\pp$ because of endogeneity of $W_i$.

%To further develop intuition for the control function approach, consider the example where  the primary and secondary outcomes are high school graduation and third grade test scores, and the treatment is class size. Using the experimental sample we estimate the the average effect of the class size on third grade scores. We then calculate the residuals in the observational study. We may find that the residuals are larger on average for the treated individuals than for the control individuals. This suggests that the treatment assignment in the observational sample was correlated with the third grade potential outcomes, with individuals with high values for the potential outcomes more likely to be in the treatment group. We then use that information to compare high school graduation outcomes for individuals with the same residuals, so we adjust for the original non-random selection into treatment.

\iffalse
\subsubsection{A Caveat on Estimation/Measurement Error in the Control Function Approach}
To see that \(\alpha^\pps_i\) must be measured without error, for expositional purpose take out the auxiliary covariates from the above setup and consider the regression
\[
Y^{\pps}_i = W_i\, \tau^\pps + \alpha^\pps_i,
\]
The fitted values from this regression are
\[
\hat{Y}^{\pps}_i = W_i\, \hat{\tau}^\pps,
\]
and the residual—used as the control function—is computed as
\[
\hat{\alpha}^\pps_i = Y^{\pps}_i - W_i\, \hat{\tau}^\pps.
\]
Thus, \(\hat{\alpha}^\pps_i\) is intended to proxy \(\alpha^\pps_i\).

In the observational sample (\(G_i = \ppo\)), the structural equation for the primary outcome is given by
\[
Y^{\pp}_i = W_i\, \tau^\pp + \alpha^\pp_i,
\]
and we assume the unobservables satisfy
\[
\alpha^\pp_i = \delta\, \alpha^\pps_i + \varepsilon^\pp_i, \quad \text{with} \quad \varepsilon^\pp_i \perp W_i \mid \alpha^\pps_i.
\]
Substituting for \(\alpha^\pp_i\) yields
\[
Y^{\pp}_i = W_i\, \tau^\pp + \delta\, \alpha^\pps_i + \varepsilon^\pp_i.
\]
Since only an estimate \(\hat{\alpha}^\pps_i\) is available, we decompose
\[
\alpha^\pps_i = \hat{\alpha}^\pps_i + \left(\alpha^\pps_i - \hat{\alpha}^\pps_i\right),
\]
which gives
\[
Y^{\pp}_i = W_i\, \tau^\pp + \delta\, \hat{\alpha}^\pps_i + \underbrace{\left[\varepsilon^\pp_i + \delta\, \left(\alpha^\pps_i - \hat{\alpha}^\pps_i\right)\right]}_{u_i}.
\]
Thus, the primary outcome equation can be written as
\[
Y^{\pp}_i = W_i\, \tau^\pp + \delta\, \hat{\alpha}^\pps_i + u_i,
\]
with the composite error term
\[
u_i = \varepsilon^\pp_i + \delta\, \left(\alpha^\pps_i - \hat{\alpha}^\pps_i\right).
\]

For the OLS estimator of \(\tau^\pp\) to be consistent, the regressors \(W_i\) and \(\hat{\alpha}^\pps_i\) must be uncorrelated with \(u_i\). However, if \(\hat{\alpha}^\pps_i\) does not perfectly recover \(\alpha^\pps_i\), the term \(\alpha^\pps_i - \hat{\alpha}^\pps_i\) introduces measurement error that induces correlation between \(\hat{\alpha}^\pps_i\) and \(u_i\).

Hence, for the control function approach to yield a consistent estimator of \(\tau^\pp\), it is crucial that \(\hat{\alpha}^\pps_i\) be measured without error. In other words, any deviation of observed test scores from their predicted values must solely reflect the latent selection component influencing the long-term outcome, rather than random measurement noise. For example, if students in small classes score unusually poorly, such deviations should be attributable to underlying unobservables affecting both test scores and high school graduation rates—not merely to idiosyncratic test-day fluctuations.
\fi

\iffalse
\subsection{An Imputation Aproach in a Linear Model Setting}
\label{section:imputation}

In a preview of a second estimation strategy consider the imputation of $Y^\pp_i$ for  units in the experimental sample given the same linear model as in the previous section. 
Substituting for $\alpha^\pps_i$ using Equation (\ref{alpha}) into Equation (\ref{control}) implies that we can write for the primary outcome in the observational sample:
\[ Y^{\pp}_i=W_i\beta+X_i^\top\lambda+\delta Y^\pps_i+\varepsilon_i,\]
where
\[ \beta=\tau^\pp-\delta\tau^\pps,\hskip1cm{\rm and}\ \  \lambda=\gamma^\pp-\delta\gamma^\pps.\]
Hence the imputed value  for $Y^\pp_i$ in the experimental sample using the estimated parameters from the observational sample leads to (ignoring estimating error)
\[ \hat  Y^{\pp}_i=W_i\beta+X_i^\top\lambda+\delta Y^\pps_i.\]
Given these imputed values we regress the longterm outcome on the covariates and the treatment in the experimental sample.
Using the omitted variable bias formula it is easy to see that  this leads to
\[ \hat Y^\pp_i=W_i\bar \beta+X_i^\top\bar \lambda+\varepsilon_i,\hskip1cm {\rm
with}\ \ 
 \bar\beta=\beta+\delta\beta^\pps=\tau^\pp.\]
Thus, the coefficient on $W_i$ in this regression of the imputed primary outcome on the treatment and the pretreatment variables, in the experimental sample, is consistent for the causal effect of the treatment on the primary outcome.
\fi

==> to_do.tex <==

\iffalse
\listoftodos
\vskip1cm
\centerline{to do's from 4/23 call}
\begin{enumerate}
\item
regarding long time lags motivation…what is a bit odd about
that motivation for the ESC estimator is that you do need a dataset
where you observe both W and Y\_P together (unlike surrogacy).  So it
can’t be purely a timing/lag motivation. I wonder if a stronger
motivation is along the lines of the abstract – there’s lots of
observational data where we observe all relevant info, but dealing
with selection is hard.

Improve motivation, vis a vis surrogate paper. Surrogate motivation is starting with experiment and using observational data to get to long run. Here motivation is observational data, using experimental data to fix biases. Also edit part about additional information in our data.

{\bf done, Raj.}

\item intro: we mention four estimation approaches – but we don’t cover
them in the main text. Do we want to edit this writing?  Also, will
move footnote 1 to results section – seems too detailed for intro.

{\bf done, guido}

\item Section 2: Latent unconfoundedness requires that all variation in
kids' test scores is due to latent unobservables that affect HS grad
rates as well, not b/c they of random factors that affect test
performance (illness, noise, etc.). In practice, we think there is
some noise in test scores, but test-retest reliability is very high
(0.9), so the noise is minor – which is probably why the ESC works in
our application. But in other settings noise in the intermediate
outcome seems more likely. Is it worth noting somewhere that 2SLS
could be used to adjust for this measurement error and get an unbiased
estimate again? Seems like a very strong assumption to require that
there is no noise in Y\_S at all.

{\bf done, guido}

\item Cost calculation: Our estimate implies that getting one more
student to graduate from high school will cost approximately \$757,000
in expenditures on class size reduction in 3rd grade (details below).
Should we include this or just say “25\% reduction in class size in a
single grade increases graduation rates by 0.71 pp”?  Or an
elasticity, e.g., 10\% reduction in class size in a single grade
increases HS graduation rates by 0.5\%?

Details: average expenditures were \$21,500 in 2020 (in 2024 dollars)
per public school pupil (NCES XX). Krueger (1999) argues that the
costs of class size reduction are approximately proportion to average
expenditures per pupil.  Reducing class size by 25\% (the average class
size reduction in the NYC data) would therefore cost \$5,375 per
student. Our estimate that a 25\% reduction in class size leads to a
0.71 pp increase in graduation rates implies that we need to treat 140
students to get one more student to graduate, which would cost
\$5,375x140 = \$757,000.

{\bf done, Raj. }

\item  put Figures 4 and 5 in appendix?

{\bf keep them in. nothing to do}

\item References to econometric work in conclusion – don’t want to cite
stuff that has already extended this?

{\bf done, guido}

\item  Abstract: shorten? Note on last sentence on covariates:
implication is that we can correct for selection that you can’t fix
w/standard observables rather than robustness?

{\bf Shorter would be better. Susan/raj take a stab at this}

\item discuss fully interacted spec with controls to add to Fig 3

{\bf done, Yechan}

\item School leaving results – how did this now become statistically sig
(in Appx Table)? Magnitude is not trivial relative to effect on HS
grad rate…need to figure this out 

{\bf done, Raj}
\end{enumerate}

\newpage

\fi


%Note: what do you get in terms of robustness by having  the $X'$ adjust for shorter term differences. Can we formalize that?

\listoftodos

\guido{discuss which journal to submit to: current decision: AER (santos), second choice JPE (Molinari).
Santos may like the semiparametric stuff. Molinari may like the selection stuff and the fact that all three of us have published little in the JPE.
}
\guido{reconstruct graph, add surrogate estimates to that}
\guido{clean up semiparametric section, add influence function estimator, discuss chen-ritzwoller}
\guido{using multiple secondary outcomes as sensitivity analyses}
\susan{sensivity analyses, bounds}
\yechan{discuss external validity assumption /comparability assumption}
\guido[is table 1 adjusted for covariates or raw means?]
